Personalization as Inverse Planning: Learning Latent Design Intents for Agentic Slide Generation via Structural Denoising

Slide design requires personalizing both deck themes and page layouts. Yet, current AI agent-based methods struggle with fine-grained, page-level design. Solely relying on prespecified templates or user verbose instructions, they fail to capture latent design intents, leaving Page-level Slide Personalization (PSP) unresolved. To close this gap, this work formulates PSP as an inverse planning problem. We propose to learn a design intent without assuming any knowledge of the specific executing tools (e.g., PowerPoint, Beamer) being used. However, relinquishing control over these tools makes the problem intractable to optimize end-to-end. To overcome this, we propose SPIRE, a principled framework to solve PSP approximately. By intentionally corrupting the visual structures of clean slides, SPIRE creates a verifiable task to denoise the corruption, whereby two agents learn to collaboratively refine executable designs via reinforcement learning (RL). We present a proof that structural denoising is a consistent surrogate for PSP, and that the multi-agent formulation strictly reduces policy gradient variance in RL. Extensive experiments demonstrate the superiority of SPIRE.

==> tables/fig_main_full.tex <==

\ExplSyntaxOn
\cs_set:Npn \loadimage #1#2#3#4 {
    \seq_clear:N \l_tmpa_seq
    \int_step_inline:nnn {#3} {#3 + #4 - 1} {
        \file_if_exist:nTF {#1/##1.pdf}
        {
            \seq_put_right:Nx \l_tmpa_seq {
                \exp_not:N \includegraphics
                    [\exp_not:n {#2}]
                    {#1/##1.pdf}
            }
        }
        {
            \seq_put_right:Nx \l_tmpa_seq {
                \exp_not:N \includegraphics
                    [\exp_not:n {#2}]
                    {example-image-a}
            }
        }
    }
    \seq_use:Nn \l_tmpa_seq {&}
}

\cs_set:Npn \calctotalwidth #1#2 {
    \fp_eval:n {
        (#2) * (#1) + (#2 - 1) * (\tabcolsep)
    } pt
}
\ExplSyntaxOff

% ========================================== %

\begin{figure*}[htb!]
\centering
\renewcommand{\tabcolsep}{1.5pt}
\def\figwidth{0.12\linewidth}
\newcommand{\rowlabel}[1]{
\adjustbox{rotate=90}{\parbox{2.5cm}{ \bf \small \centering #1}}
}

\begin{tabular}{c ccccc cc} 
\toprule[0.4ex]

\small Ref & \small AutoPre. & \small PPTAgent & \small SD 3.5 & \small o4-mini& \small base & \small Ours & \small Gold \\
\noalign{\vskip 0.5ex}
\midrule[0.2ex]

\loadimage{figures/93_s_152_9}{width=\figwidth}{0}{8} \\ 
\loadimage{figures/12_s_122_53}{width=\figwidth}{0}{8} \\
\loadimage{figures/63_s_115_8}{width=\figwidth}{0}{8} \\
\loadimage{figures/93_s_152_9}{width=\figwidth}{0}{8} \\

\loadimage{figures/social_media_21}{width=\figwidth}{0}{8} \\
\loadimage{figures/business_2}{width=\figwidth}{0}{8} \\
\loadimage{figures/entrepreneur_3}{width=\figwidth}{0}{8} \\

\bottomrule[0.4ex]
\end{tabular}
\caption{
Qualitative comparison of slide generation results.
}
\label{fig:main}
\end{figure*}




